Modeling magnetospheric fields in the Jupiter system

The various processes which generate magnetic fields within the Jupiter system are exemplary for a large class of similar processes occurring at other planets in the solar system, but also around extrasolar planets. Jupiter's large internal dynamo magnetic field generates a gigantic magnetosphere, which is strongly rotational driven and possesses large plasma sources located deeply within the magnetosphere. The combination of the latter two effects is the primary reason for Jupiter's main auroral ovals. Jupiter's moon Ganymede is the only known moon with an intrinsic dynamo magnetic field, which generates a mini-magnetosphere located within Jupiter's larger magnetosphere including two auroral ovals. Ganymede's magnetosphere is qualitatively different compared to the one from Jupiter. It possesses no bow shock but develops Alfv\'en wings similar to most of the extrasolar planets which orbit their host stars within 0.1 AU. New numerical models of Jupiter's and Ganymede's magnetospheres presented here provide quantitative insight into the processes that maintain these magnetospheres. Jupiter's magnetospheric field is approximately time-periodic at the locations of Jupiter's moons and induces secondary magnetic fields in electrically conductive layers such as subsurface oceans. In the case of Ganymede, these secondary magnetic fields influence the oscillation of the location of its auroral ovals. Based on dedicated Hubble Space Telescope observations, an analysis of the amplitudes of the auroral oscillations provides evidence that Ganymede harbors a subsurface ocean. Callisto in contrast does not possess a mini-magnetosphere, but still shows a perturbed magnetic field environment. Callisto's ionosphere and atmospheric UV emission is different compared to the other Galilean satellites as it is primarily been generated by solar photons compared to magnetospheric electrons.

==> reference_saur.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use

\bibliographystyle{spbasic}
%\bibliographystyle{agu}
%\bibliographystyle{natbib}
\bibliography{../../../../../../Forschung/literatur/lit.bib}
%

